Provable Dynamic Fusion for Low-Quality Multimodal Data

The inherent challenge of multimodal fusion is to precisely capture the cross-modal correlation and flexibly conduct cross-modal interaction. To fully release the value of each modality and mitigate the influence of low-quality multimodal data, dynamic multimodal fusion emerges as a promising learning paradigm. Despite its widespread use, theoretical justifications in this field are still notably lacking. Can we design a provably robust multimodal fusion method? This paper provides theoretical understandings to answer this question under a most popular multimodal fusion framework from the generalization perspective. We proceed to reveal that several uncertainty estimation solutions are naturally available to achieve robust multimodal fusion. Then a novel multimodal fusion framework termed Quality-aware Multimodal Fusion (QMF) is proposed, which can improve the performance in terms of classification accuracy and model robustness. Extensive experimental results on multiple benchmarks can support our findings.

==> tab-noise-nyud2.tex <==
\begin{table*}[!t]
\small
\vspace{1mm}
% \vskip 0.35in
\begin{center}
% \begin{spacing}{1.05}   
\caption{Classification accuracy performance comparison on \textbf{NYUD2} dataset when 50\% of the modalities is corrupted with Gaussian noise (i.e., zero mean with varying variance $\epsilon$).}
%\label{tab:nyud2-sys-noise}
\center
{
% \setlength{\tabcolsep}{1.9mm}
\begin{tabular}{c|c|c|ccccc}
\toprule
\multicolumn{1}{c}{\text{Modality}}  & \multicolumn{1}{c}{\text{Method}}  & \multicolumn{1}{c}{\text{QMF}}  &
\text{$\mathbf{\epsilon=0.0}$}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=10.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=20.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=30.0}$\\ \end{tabular}}
\\ \midrule
{\text{RGB}}  
    &   \multirow{2}{*}{\text{Uni-modal}}      & \xmark                                         &${63.42\pm0.69}$  
       &${45.78\pm1.17}$   
       &${39.48\pm2.01}$
       &${38.59\pm1.94}$ \\
                                                                             {\text{Depth}}      &  & \xmark            
                                                         &${62.14\pm1.40}$   
                                                         &${45.14\pm2.92}$   
                                                         &${37.37\pm3.25}$ 
                                                         &${35.72\pm2.23}$                                    \\ \midrule \multirow{8}{*} {\text{RGB-D}}
      &  \multirow{3}{*}{\text{LF}}       & \xmark                                                    &$69.11\pm0.72$  &$52.69\pm2.58$   &$43.91\pm2.48$   &$41.53\pm2.51$    \\
                                                                                  
                                                            &                           & \cmark                                                                                            &${70.86\pm0.96}$   &${57.86\pm1.94}$   &${53.27\pm2.95}$  &${52.08\pm3.27}$   \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.25 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.17 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 9.36 $}}  & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.55 $}}                                     \\ \cmidrule{2-7}
     &  \multirow{3}{*}{\text{Align}}      & \xmark                                                      &${71.19\pm1.49}$  &${53.79\pm2.60}$  &${47.40\pm1.56}$  &${45.84\pm2.25}$                                         \\
                                                                                 &             & \cmark                                                       &${70.76\pm0.38}$  &${59.24\pm1.50}$   &${53.36\pm0.72}$         &${53.21\pm1.12}$                        \\& & Improve & \textcolor{mycolor1}{{$~~~~~~~~\bigtriangledown 0.43 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.55 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.96 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.47 $}}                                                                              \\\cmidrule{2-7}
     &  \multirow{3}{*}{\text{MMTM}}      & \xmark                                                      &${71.04\pm0.16}$  &${51.80\pm3.70}$  &${45.75\pm3.41}$  &${43.64\pm2.36}$                                         \\
                                                                                 &             & \cmark                                                       &${69.39\pm0.53}$  &${60.31\pm0.78}$   &${55.78\pm1.41}$         &${54.46\pm1.74}$                        \\& & Improve & \textcolor{mycolor1}{{$~~~~~~~~\bigtriangledown 1.65 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 8.51 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.03 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.82 $}}\\  \bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\vspace{1mm}
\end{table*}





==> tabs/tab-classification.tex <==
\begin{table*}[!t]
\small
\vspace{0.0cm}
% \vskip 0.35in
\begin{center}
% \begin{spacing}{1.05}   
\caption{Classification comparison when 50\% of the modalities are corrupted with Gaussian noise.}
%\label{tab:classification}
\center
{
% \setlength{\tabcolsep}{1.9mm}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{c|c|c|c|cccccc}
\toprule
\multicolumn{1}{c}{\text{Dataset}}  &\multicolumn{1}{c}{\text{Modality}}  & \multicolumn{1}{c}{\text{Method}}  & \multicolumn{1}{c}{\text{QMF}}  &
\text{$\mathbf{\epsilon=0.0}$}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=5.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=10.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=20.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=30.0}$\\ \end{tabular}}
\\ \toprule
 \multirow{12}{*} {\text{NYUD2}} & {\text{RGB}}  
    &   \multirow{2}{*}{\text{Uni-modal}}      & \xmark                                         &${63.42\pm0.69}$  &${53.30\pm0.81}$
       &${45.78\pm1.17}$   
       &${39.48\pm2.01}$
       &${38.59\pm1.94}$ \\
                                                                     &        {\text{Depth}}      &  & \xmark            
                                                         &${62.14\pm1.40}$   
                                                         &${52.51\pm1.72}$   
                                                         &${45.14\pm2.92}$   
                                                         &${37.37\pm3.25}$ 
                                                         &${35.72\pm2.23}$                                    \\ \cline{2-9} & \multirow{11}{*} {\text{RGB-D}}
      &  \multirow{3}{*}{\text{Late fusion}}       & \xmark                                                    &$69.11\pm0.72$ &$60.58\pm1.53$ &$52.69\pm2.58$   &$43.91\pm2.48$   &$41.53\pm2.51$    \\
                                                                                  
                                                 &           &                           & \cmark                                                                                            &${70.86\pm0.96}$   &${63.64\pm1.22}$ &${57.86\pm1.94}$   &${53.27\pm2.95}$  &${52.08\pm3.27}$   \\& & & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 1.75 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.06 $}}&\textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.17 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 9.36 $}}  & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.55 $}}                               \\\cline{3-9}
&     &  \multirow{3}{*}{\text{Concatenate}}      & \xmark                                                      &${70.12\pm0.39}$  &${61.25\pm1.91}$ &${54.40\pm3.60}$  &${47.06\pm3.75}$  &${45.23\pm3.84}$                                         \\
                                                                   &              &             & \cmark                                                       &${70.00\pm0.39}$  &${63.52\pm0.86}$ &${59.42\pm1.08}$   &${54.01\pm1.94}$         &${52.63\pm2.23}$                        \\& & & Improve & - & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 2.27 $}}&\textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.02 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.95 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.40 $}}      \\  \cline{3-9}
    & &  \multirow{3}{*}{\text{Align}}      & \xmark                                                      &${71.19\pm1.49}$  &${60.40\pm1.62}$ &${53.79\pm2.60}$  &${47.40\pm1.56}$  &${45.84\pm2.25}$                                         \\
                                                                            &     &             & \cmark                                                       &${71.13\pm0.38}$ &${63.94\pm0.83}$  &${59.24\pm1.50}$   &${53.36\pm0.72}$         &${53.21\pm1.12}$                        \\& & & Improve & - & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.54 $}}&\textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.55 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.96 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.47 $}}                                                                              \\ \cline{3-9}
&     &  \multirow{3}{*}{\text{MMTM}}      & \xmark                                                      &${71.04\pm0.16}$ &${59.91\pm2.25}$ &${51.80\pm3.70}$  &${45.75\pm3.41}$  &${43.64\pm2.36}$                                         \\
                                                                   &              &             & \cmark                                                       &${71.25\pm0.31}$ &${64.68\pm0.77}$ &${60.31\pm0.78}$   &${55.78\pm1.41}$         &${54.46\pm1.74}$                        \\& & & Improve & - & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 4.77 $}} &\textcolor{mycolor2}{{$~~~~~~\bigtriangleup 8.51 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.03 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.82 $}}\\ \midrule  \multirow{12}{*} {\text{SUN}} & {\text{RGB}}  
    &   \multirow{2}{*}{\text{Uni-modal}}      & \xmark                                         &${57.49\pm0.58}$  
    &${49.13\pm0.44}$
       &${43.51\pm0.77}$   
       &${39.61\pm0.98}$
       &${37.29\pm0.87}$ \\
                                                                     &        {\text{Depth}}      &  & \xmark            
                                                         &${53.88\pm0.57}$
                                                         &${38.52\pm1.84}$
                                                         &${33.31\pm1.63}$   
                                                         &${29.33\pm0.33}$ 
                                                         &${28.46\pm0.12}$                                    \\ \cline{2-9} & \multirow{11}{*} {\text{RGB-D}}
      &  \multirow{3}{*}{\text{Late fusion}}       & \xmark                                                   &$62.00\pm0.15$  &$52.52\pm0.67$ &$47.48\pm1.40$   &$43.21\pm2.21$   &$41.63\pm2.63$    \\
                                                                                  
                                                 &           &                           & \cmark                                                                                            &${62.22\pm0.34}$   &${55.06\pm0.67}$ &${50.66\pm1.13}$   &${46.35\pm1.67}$  &${43.05\pm1.69}$   \\& & & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.22 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 2.54 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.12 $}}  & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.14 $}}     & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 2.42 $}}                           \\\cline{3-9}
&     &  \multirow{3}{*}{\text{Concatenate}}      & \xmark                                                      &${62.48\pm0.50}$  &${53.30\pm0.39}$ &${48.01\pm0.96}$  &${41.85\pm3.11}$  &${38.70\pm4.65}$                                         \\
                                                                   &              &             & \cmark                                                       &${61.90\pm0.40}$  &${55.33\pm0.32}$ &${51.23\pm0.62}$  &${47.98\pm1.03}$  &${45.47\pm1.45}$                        \\& & & Improve & \textcolor{mycolor1}{{$~~~~~~~~\bigtriangledown 0.58 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 2.03 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.22 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.13 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.63 $}}      \\  \cline{3-9}
    & &  \multirow{3}{*}{\text{Align}}      & \xmark                                                      &${61.22\pm0.66}$  &${49.66\pm1.40}$ &${43.96\pm1.98}$  &${39.79\pm1.34}$  &${38.69\pm1.06}$                                         \\
                                                                            &     &             & \cmark                                                       &${62.13\pm0.44}$
                                                                            &${55.45\pm0.98}$ &${50.92\pm1.32}$   &${48.18\pm0.72}$         &${45.87\pm1.63}$                        \\& & & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.91 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.79 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.98 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup6.39 $}} &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.18 $}}                                                                              \\ \cline{3-9}
&     &  \multirow{3}{*}{\text{MMTM}}      & \xmark                                                      &${61.72\pm0.67}$  &${51.86\pm1.14}$ &${46.03\pm1.47}$  &${41.19\pm1.59}$  &${39.50\pm2.47}$                                         \\
                                                                   &              &             & \cmark                                                       &${62.70\pm0.30}$
                                                                   &${55.93\pm1.04}$
                                                                   &${51.65\pm1.59}$   &${48.78\pm1.34}$         &${46.45\pm0.67}$                       \\& & & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.98 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 4.07 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 5.62 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.59 $}} &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.95 $}}\\


\bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\vspace{0mm}
\end{table*}





==> tabs/tab-dynamic-interaction.tex <==

\begin{table*}[!h]
\vspace{1mm}
% \vskip 0.35in
\begin{center}
% \begin{spacing}{1.05}
\caption{Weighted cross-modal interaction}
%\label{tab:dynamic interaction}
\center
\resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{1.9mm}
\begin{tabular}{c|c|c}
\toprule
{\tabincell{c}{\textbf{Type} \\ }}  & {\textbf{Origin} }  & {\tabincell{c}{\textbf{QMI} \\}}\\

\midrule
        I
       & $h=F(h^A,h^B)$
       & $h=F(h^A*QAC^{A/B},h^B*QAC^{B/A})$ \\ \midrule
       II & $\left\{             \begin{array}{lr}             h_A^*=G_B(h^B)&  \\             h_B^*=G_A(h^A)&               \end{array}\right.$&$\left\{             \begin{array}{lr}             h_A^*=h_A\cdot G_B(h^B*QAC^{B/A})&  \\             h_B^*=h_B\cdot G_A(h^A*QAC^{A/B})&               \end{array}\right.$\\
       \bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\vspace{1mm}
\end{table*}





==> tabs/tab-noise-sun.tex <==
\begin{table*}[!htbp]
\vspace{1mm}
% \vskip 0.35in
\begin{center}
% \begin{spacing}{1.05}   
\caption{Classification accuracy performance comparison on \textbf{SUN-RGBD} dataset when 50\% of the modalities is corrupted with Gaussian noise (i.e., zero mean with varying variance $\epsilon$).}
%\label{tab:sun-sys-noise}
\center
\resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{1.9mm}
\begin{tabular}{c|c|c|ccccc}
\toprule
\multicolumn{1}{c}{\text{Modality}}  & \multicolumn{1}{c}{\text{Method}}  & \multicolumn{1}{c}{\text{QMI}}  &
\text{$\mathbf{\epsilon=0.0}$}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=10.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=20.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=30.0}$\\ \end{tabular}}
\\ \midrule
{\text{RGB}}  
    &   \multirow{2}{*}{\text{Uni-modal}}      & \xmark                                         &${57.49\pm0.58}$  
       &${43.51\pm0.77}$   
       &${39.61\pm0.98}$
       &${37.29\pm0.87}$ \\
                                                                             {\text{Depth}}      &  & \xmark            
                                                         &${53.88\pm0.57}$   
                                                         &${33.31\pm1.63}$   
                                                         &${29.33\pm0.33}$ 
                                                         &${28.46\pm0.12}$                                    \\ \midrule \multirow{8}{*} {\text{RGB-D}}
      &  \multirow{3}{*}{\text{LF}}       & \xmark                                                    &$62.00\pm0.15$  &$47.48\pm1.40$   &$43.21\pm2.21$   &$41.63\pm2.63$    \\
                                                                                  
                                                            &                           & \cmark                                                                                            &${62.22\pm0.34}$   &${50.66\pm1.13}$   &${46.35\pm1.67}$  &${43.05\pm1.69}$   \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.22 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.18 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.24 $}}  & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 1.42 $}}                                     \\ \cmidrule{2-7}
     &  \multirow{3}{*}{\text{Align}}      & \xmark                                                      &${61.22\pm0.66}$  &${43.96\pm1.98}$  &${39.79\pm1.34}$  &${38.69\pm1.06}$                                         \\
                                                                                 &             & \cmark                                                       &${62.13\pm0.44}$  &${50.92\pm1.32}$   &${48.18\pm0.72}$         &${45.87\pm1.63}$                        \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.91 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.96 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 8.39 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.18 $}}                                                                              \\\cmidrule{2-7}
     &  \multirow{3}{*}{\text{MMTM}}      & \xmark                                                      &${61.72\pm0.67}$  &${46.03\pm1.47}$  &${41.19\pm1.59}$  &${39.50\pm2.47}$                                         \\
                                                                                 &             & \cmark                                                       &${61.18\pm0.42}$  &${50.69\pm1.50}$   &${48.61\pm1.06}$         &${46.98\pm0.70}$                        \\& & Improve & \textcolor{mycolor1}{{$~~~~~~~~\bigtriangledown 0.54 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 4.66 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.42 $}}  &  \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 7.48 $}}\\  \bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\vspace{1mm}
\end{table*}





==> tabs/tab-nyud2-seg.tex <==
\begin{table*}[!htbp]\scriptsize
\vspace{-20mm}
% \vskip 0.35in
\begin{center}
% \begin{spacing}{1.05}   
\caption{Mean intersection over union (MIoU) comparison on \textbf{NYUD2} dataset when 50\% of the modalities is corrupted with Gaussian noise (i.e., zero mean with varying variance $\epsilon$).}
%\label{tab:nyud2-segmentation-noise}
\center

\resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{1.9mm}
\begin{tabular}{c|c|c|ccccc}
\toprule
\multicolumn{1}{c}{\text{Modality}}  & \multicolumn{1}{c}{\text{Method}}  & \multicolumn{1}{c}{\text{QMF}}  &
\text{$\mathbf{\epsilon=0.0}$}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=10.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=20.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=30.0}$\\ \end{tabular}}
\\ \midrule
{\text{RGB}}  
    &   \multirow{2}{*}{\text{Uni-modal}}      & \xmark                                         &${43.42}$  
       &${45.78}$   
       &${39.48}$
       &${38.59}$ \\
                                                                             {\text{Depth}}      &  & \xmark            
                                                         &${62.14}$   
                                                         &${45.14}$   
                                                         &${37.37}$ 
                                                         &${35.72}$                                    \\ \midrule \multirow{8}{*} {\text{RGB-D}}
      &  \multirow{3}{*}{\text{add}}       & \xmark                                                    &$48.62$  &$40.43$   &$31.63$   &$28.74$    \\
                                                                                  
                                                            &                           & \cmark                                                                                            &${49.51}$   &${46.67}$   &${42.70}$  &${39.66}$   \\& & Improve & \textcolor{mycolor2}{{$\bigtriangleup 0.89 $}} & \textcolor{mycolor2}{{$\bigtriangleup 6.24 $}}& \textcolor{mycolor2}{{$\bigtriangleup 11.07 $}}  & \textcolor{mycolor2}{{$\bigtriangleup 10.92 $}}                                     \\ \cmidrule{2-7}
     &  \multirow{3}{*}{\text{SE-add}}      & \xmark                                                      &${48.77}$  &${40.51}$  &${47.40}$  &${45.84}$                                         \\
                                                                                 &             & \cmark                                                       &${70.76}$  &${59.24}$   &${53.36}$         &${53.21}$                        \\& & Improve & \textcolor{mycolor1}{{$\bigtriangledown 0.43 $}} & \textcolor{mycolor2}{{$\bigtriangleup 5.55 $}}& \textcolor{mycolor2}{{$\bigtriangleup 5.96 $}}  &  \textcolor{mycolor2}{{$\bigtriangleup 7.47 $}}                                                                              \\\cmidrule{2-7}
     &  \multirow{3}{*}{\text{ESA-Net}}      & \xmark                                                      &${71.04}$  &${51.80}$  &${45.75}$  &${43.64}$                                         \\
                                                                                 &             & \cmark                                                       &${69.39}$  &${60.31}$   &${55.78}$         &${54.46}$                        \\& & Improve & \textcolor{mycolor1}{{$\bigtriangledown 1.65 $}} & \textcolor{mycolor2}{{$\bigtriangleup 8.51 $}}& \textcolor{mycolor2}{{$\bigtriangleup 10.03 $}}  &  \textcolor{mycolor2}{{$\bigtriangleup 10.82 $}}\\  \bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\vspace{1mm}
\end{table*}





==> tabs/tab-seg.tex <==
\begin{table*}[!htbp]
\small
%\vspace{-0.5cm}

% \vskip 0.35in
\begin{center}
% \begin{spacing}{1.05}   
\caption{Comparison on \textbf{NYUD2} in terms of MIoU  when 50\% of the modalities is corrupted with Gaussian noise.}
\vspace{0.3cm}
%\label{tab:nyud2-segmentation-noise}
\center
{
%\setlength{\tabcolsep}{1.9mm}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{c|c|c|c|cccccc}
\toprule
\multicolumn{1}{c}{\text{Dataset}}  &\multicolumn{1}{c}{\text{Modality}}  & \multicolumn{1}{c}{\text{Method}}  & \multicolumn{1}{c}{\text{QMI}}  &
\text{$\mathbf{\epsilon=0.0}$}& \text{\begin{tabular}[c]
{@{}c@{}}$\mathbf{\epsilon=5.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=10.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=20.0}$\\ \end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=30.0}$\\ \end{tabular}}
\\ \toprule \multirow{10}{*}{\text{NYUD2}}&
{\text{RGB}}  
    &   \multirow{2}{*}{\text{Uni-modal}}      & \xmark                                         &${42.71}$  
       &${39.72}$   
       &${33.97}$
       &${26.33}$
       &${25.27}$ \\&
                                                                             {\text{Depth}}      &  & \xmark            
                                                         &${40.08}$   
                                                         &${33.42}$   
                                                         &${26.35}$ 
                                                         &${25.06}$
                                                         &${21.77}$                                    \\ \cline{2-9} & \multirow{8}{*} {\text{RGB-D}}
      &  \multirow{3}{*}{\text{Late fusion}}       & \xmark                                                    &$42.76$  &$38.54$   &$31.94$   &$24.46$ &$22.34$   \\
                                                                                  
                                                            &  &                         & \cmark                                                                                            &${46.24}$   &${44.88}$   &${43.01}$  &${40.35}$
                                                            &${38.03}$ 
                                                            \\& & & Improve & \textcolor{mycolor2}{{$\bigtriangleup 3.48 $}} & \textcolor{mycolor2}{{$\bigtriangleup 6.34 $}}&
                                                            \textcolor{mycolor2}{{$\bigtriangleup 11.07 $}}  &
                                                            \textcolor{mycolor2}{{$\bigtriangleup 15.89 $}}  & \textcolor{mycolor2}{{$\bigtriangleup 15.69 $}}                                     \\ \cline{3-9}
  &   &  \multirow{3}{*}{\text{SE-add}}      & \xmark                                                      &${48.77}$  &${43.82}$  &${40.51}$  &${34.74}$   &${29.53}$                                         \\&
                                                                                 &             & \cmark                                                       &${48.46}$  &${47.43}$   &${46.37}$         &${43.60}$   &${39.52}$                      \\& & & Improve & \textcolor{mycolor1}{{$\bigtriangledown 0.31 $}} & \textcolor{mycolor2}{{$\bigtriangleup 3.61 $}}& \textcolor{mycolor2}{{$\bigtriangleup 5.86 $}}  &  \textcolor{mycolor2}{{$\bigtriangleup 8.86 $}}  &  \textcolor{mycolor2}{{$\bigtriangleup 9.99 $}}                                                                              \\\cline{3-9}
   &  &  \multirow{3}{*}{\text{ESA-Net}}      & \xmark                                                      &${48.99}$  &${46.79}$  &${41.42}$  &${33.03}$   &${27.10}$                                \\&
                                                                                 &             & \cmark                                                       &${49.51}$  &${48.83}$   &${46.80}$         &${43.24}$ &${39.39}$           \\& & & Improve & \textcolor{mycolor2}{{$\bigtriangleup 0.52 $}} & \textcolor{mycolor2}{{$\bigtriangleup 2.04 $}}& \textcolor{mycolor2}{{$\bigtriangleup 5.38 $}}  &  \textcolor{mycolor2}{{$\bigtriangleup 10.21 $}} &
                                                                                 \textcolor{mycolor2}{{$\bigtriangleup 12.29 $}}\\  \bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\vspace{0.0mm}
\end{table*}




